Automated Machine Learning in Practice: State of the Art and Recent Results

A main driver behind the digitization of industry and society is the belief that data-driven model building and decision making can contribute to higher degrees of automation and more informed decisions. Building such models from data often involves the application of some form of machine learning. Thus, there is an ever growing demand in work force with the necessary skill set to do so. This demand has given rise to a new research topic concerned with fitting machine learning models fully automatically - AutoML. This paper gives an overview of the state of the art in AutoML with a focus on practical applicability in a business context, and provides recent benchmark results on the most important AutoML algorithms.

==> table2.tex <==
\begin{tabular}{l l l| c c c c c c c c c|cc}
		\toprule[1.5pt]
		& & &  \multicolumn{3}{c}{\head{DSM}} & \multicolumn{3}{c}{\head{Auto-Sklearn}} &
		\multicolumn{3}{c}{\head{TPOT}} & \multicolumn{2}{c}{\head{Portfolio Hyperband}} \\
		\textbf{Dataset} & \textbf{Task} & \textbf{Metric} & \normal{\head{Validation}} &
		\textbf{Test} & \textbf{Time} & \textbf{Validation} & \textbf{Test} & \textbf{Time} & \textbf{Validation} &  \textbf{Test} & \textbf{Time}  & \textbf{Test, full time} & \textbf{Test, 10 Min} \\
		\cmidrule(lr){1-14}  

Cadata        & Regression                   & R2 (coefficient of determination)   &        0.7078        &        0.7119        &      55.0    &        0.7571        &        0.7327        &      54.9       &        \textbf{0.8247}        &        \textbf{0.7989}        &      54.6              & - & - \\ 
Christine     & Binary classification        & Balanced accuracy score  &        0.7362        &        0.7146        &      99.4              &        0.7251        &        0.7392        &      99.3       &        0.7325        &        0.7442        &      105.1           & \textbf{0.753} & \textbf{0.744}   \\ 
Digits        & Multiclass classification    & Balanced accuracy score   &        0.8900        &        0.8751        &      201.2              &        \textbf{0.9540}        &        \textbf{0.9542}        &      201.2      &        0.9520        &        0.9476        &      207.2       & - & -   \\ 
Fabert        & Multiclass classification    & Accuracy score    &        0.8883        &        0.8665        &      77.5                       &        0.8871        &        \textbf{0.8908}        &      77.4       &        \textbf{0.8920}        &        0.8835        &      78.5       & - & -    \\ 
Helena        & Multiclass classification    & Balanced accuracy score    &        0.2085        &        0.2103        &      190.2             &        0.3221        &        0.3235        &      216.4      &        \textbf{0.3505}        &        \textbf{0.3470}        &      197.5       & - & -   \\ 
Jasmine       & Binary classification        & Balanced accuracy score    &        0.8020        &        \textbf{0.8371}        &      24.1             &        \textbf{0.8154}        &        0.8214        &      24.0       &        0.7886        &        0.8326        &      25.9         & - & -   \\ 
Madeline      & Binary classification        & Balanced accuracy score   &        0.7707        &        0.7686        &      48.3                &        \textbf{0.8822}        &        \textbf{0.8896}        &      48.2       &        0.8567        &        0.8684        &      53.0        & 0.868 & 0.848  \\ 
Philippine    & Binary classification        & Balanced accuracy score      &        0.7581        &        0.7406        &      56.3              &        \textbf{0.7770}        &        0.7634        &      56.2       &        0.7616        &        \textbf{0.7703}        &      56.4       & 0.741 & 0.753  \\ 
Sylvine       & Binary classification        & Balanced accuracy score    &        0.9414        &        0.9233        &      28.9              &        0.9434        &        0.9350        &      28.9       &        \textbf{0.9473}        &        \textbf{0.9415}        &      29.0         & \textbf{0.947} & 0.916  \\ 
Volkert       & Multiclass classification    & Accuracy score    &        0.8143        &        0.8154        &      122.3                      &        \textbf{0.8858}        &        \textbf{0.8880}        &      122.2      &        0.8739        &        0.8720        &      125.5        & - & -  \\ 
\midrule
\multicolumn{3}{l|}{\head{Average Performance}}   &        0.7517        &        0.7463        &      \textbf{90.31} &   0.7949        &        0.7938        &      92.85      &        \textbf{0.7980}        &        \textbf{0.8006}        &      93.26        &   &    \\
		\bottomrule[1.5pt]
	\end{tabular}
